SmileSplat: Generalizable Gaussian Splats for Unconstrained Sparse Images

Sparse Multi-view Images can be Learned to predict explicit radiance fields via Generalizable Gaussian Splatting approaches, which can achieve wider application prospects in real-life when ground-truth camera parameters are not required as inputs. In this paper, a novel generalizable Gaussian Splatting method, SmileSplat, is proposed to reconstruct pixel-aligned Gaussian surfels for diverse scenarios only requiring unconstrained sparse multi-view images. First, Gaussian surfels are predicted based on the multi-head Gaussian regression decoder, which can are represented with less degree-of-freedom but have better multi-view consistency. Furthermore, the normal vectors of Gaussian surfel are enhanced based on high-quality of normal priors. Second, the Gaussians and camera parameters (both extrinsic and intrinsic) are optimized to obtain high-quality Gaussian radiance fields for novel view synthesis tasks based on the proposed Bundle-Adjusting Gaussian Splatting module. Extensive experiments on novel view rendering and depth map prediction tasks are conducted on public datasets, demonstrating that the proposed method achieves state-of-the-art performance in various 3D vision tasks. More information can be found on our project page (https://yanyan-li.github.io/project/gs/smilesplat)

==> img/fig.tex <==
\begin{figure}
    \centering
    \label{subfig:short-10-a}
    \resizebox{0.8\linewidth}{!}{
   \begin{tikzpicture}
   \begin{axis}[
       xlabel=$Pair \; ID $,
       ylabel=$PSNR$,
       xmin=0, xmax=20,
       ymin=18, ymax=50,
       xtick={2,5, 10, 15,20},
       % xticklabels={A,B,X}, % <---
       ytick={18,23,35,...,50}]
   \addplot[mark=*,blue] plot coordinates {
     (1,  30.039) 
     (2,  26.667) 
     (3,  25.074) 
     (4,  16.098) 
     (5,  24.671) 
     (6,  20.616) 
     (7,  22.437)  
     (8,  21.921 ) 
     (9,  20.689)  
     (10,  22.803) 
     (11,  15.820) 
     (12,  26.628) 
     (13,  21.434)  
     (14,  26.972) 
     (15,  21.132) 
     (16,  23.444) 
     (17,  18.270) 
     (18,  24.824) 
     (19,  24.170) 
     (20,  25.367)}; 
  \addlegendentry{View 1 Initial}
   \addplot[color=green,mark=x]
       plot coordinates {
       (1, 45.281)  
     (2,  36.444)  
     (3,  34.496)   
     (4,  22.770)  
     (5,  33.440)  
     (6,  29.035)  
     (7,  32.613)  
     (8,  28.230)  
     (9,  30.465) 
     (10,  31.327) 
     (11, 24.850)    
     (12,  33.811)  
     (13,  31.212)  
     (14,  37.682) 
     (15,  30.406) 
     (16, 34.627) 
     (17, 32.223)
     (18, 36.569) 
     (19, 38.891 ) 
     (20, 37.919)}; 
   \addlegendentry{View 1 Opti}
   \addplot[mark=*,brown] plot coordinates {
        (1,   28.311)  
     (2,   17.661)   
     (3,  16.493)   
     (4,  11.333 )  
     (5,   20.585)  
     (6,  17.490 )  
     (7,    16.063)  
     (8,  17.625)  
     (9,    12.204)  
     (10,   16.933) 
     (11,   8.549)  
     (12,   19.804)
     (13,  17.213)  
     (14,    18.005) 
     (15,   10.574) 
     (16,   17.680) 
     (17,   17.955) 
     (18,  21.849) 
     (19,   18.933) 
     (20,   21.864)};  
  \addlegendentry{View 2 Initial}
   \addplot[color=black,mark=x] plot coordinates {
        (1,  42.553)  
         (2,  22.174) 
         (3,   27.623) 
         (4,   18.853)  
         (5,   28.572)  
         (6,   31.382)  
         (7,    23.478)  
         (8,    21.305)  
         (9,    25.753) 
         (10,   22.710)
         (11,   13.222) 
         (12,    30.595) 
         (13,   24.253)
         (14,   32.820) 
         (15,    12.205)
         (16,  29.435) 
         (17, 30.530) 
         (18,  36.297) 
         (19,  37.624) 
         (20,  35.466)}; 
     \addlegendentry{View 2 Refine}
   \addplot[mark=*,blue] plot coordinates {
     (1,   29.642)
     (2,   21.962)
     (3,     20.319)
     (4,    11.319)
     (5,    18.735)
     (6,    18.486)
     (7,    16.949)
     (8,    21.360)
     (9,    12.241)
     (10,   17.577)
     (11,    8.592)
     (12,   22.656)
     (13,    15.225)
     (14,   23.943)
     (15,  18.115)
     (16,   18.746)
     (17,   19.204)
     (18,   22.215)
     (19,   23.991)
     (20,  20.978)};
  \addlegendentry{View 3 Initial}
   \addplot[color=green,mark=x]
       plot coordinates {
       (1, 38.989)
     (2,    27.363)
     (3,    25.883)
     (4,    15.103)
     (5,   22.179)
     (6,    28.485 )
     (7,    26.539)
     (8,    23.497)
     (9,    23.308)
     (10,   21.875)
     (11,  11.309)
     (12,   30.903)
     (13,    16.395)
     (14,    33.978)
     (15,    19.784)
     (16,  25.882)
     (17,  30.488)
     (18,  36.237)
     (19,  34.814)
     (20, 22.658)};
     \addlegendentry{View 3 Opti}
   \end{axis}
   \end{tikzpicture}}
    \caption{Comparison of Rendering performance in initial prediction and refinement modules. 100 pairs are randomly selected based from the Re10K dataset.}
    \label{fig:icl-10sparse}
\end{figure}
